Cheap IR Evaluation: Fewer Topics, No Relevance Judgements, and Crowdsourced Assessments

To evaluate Information Retrieval (IR) effectiveness, a possible approach is to use test collections, which are composed of a collection of documents, a set of description of information needs (called topics), and a set of relevant documents to each topic. Test collections are modelled in a competition scenario: for example, in the well known TREC initiative, participants run their own retrieval systems over a set of topics and they provide a ranked list of retrieved documents; some of the retrieved documents (usually the first ranked) constitute the so called pool, and their relevance is evaluated by human assessors; the document list is then used to compute effectiveness metrics and rank the participant systems. Private Web Search companies also run their in-house evaluation exercises; although the details are mostly unknown, and the aims are somehow different, the overall approach shares several issues with the test collection approach. The aim of this work is to: (i) develop and improve some state-of-the-art work on the evaluation of IR effectiveness while saving resources, and (ii) propose a novel, more principled and engineered, overall approach to test collection based effectiveness evaluation. [...]

==> img/IPM/Figs/APPrediction.tex <==
\begin{tabular}{l l l c l}
\begin{tabular}{ ll |c|}
         & \multicolumn{1}{c}{} & \multicolumn{1}{@{}c@{}}{$\widehat{\AP}_1^s$} \\
  \cline{3-3}    
  $s_1$  & $t_1$                &                                               \\
  \vdots & \vdots               &                                               \\
  $s_m$  & $t_1$                &                                               \\
  \cline{3-3} 
  $s_1$  & $t_2$                &                                               \\
  \vdots & \vdots               &                                               \\
  $s_m$  & $t_2$                &                                               \\
  \cline{3-3} 
  \vdots & \vdots               &                                               \\
  \cline{3-3} 
  $s_1$  & $t_n$                &                                               \\
  \vdots & \vdots               &                                               \\
  $s_m$  & $t_n$                &                                               \\
  \cline{3-3}
\end{tabular}
         & 
\begin{tabular}{@{}c@{}|c|}
 \multicolumn{1}{@{}c@{}}{}&\multicolumn{1}{@{}c@{}}{$\widehat{\AP}_i^s$}                                  \\
  \cline{2-2}    
          &                                                                      \\
  \phantom{\vdots}   &                                                                     \\
            &                                                                    \\
  \cline{2-2} 
          &                                                                      \\
  \phantom{\vdots}    &                                                                     \\
            &                                                                    \\
  \cline{2-2} 
  \phantom{\vdots}   &                                                                      \\
  \cline{2-2} 
          &                                                                      \\
  \phantom{\vdots}    &                                                                     \\
            &                                                                    \\
  \cline{2-2}
\end{tabular}
         & 
\begin{tabular}{@{}c@{}|c|}
 \multicolumn{1}{@{}c@{}}{}&\multicolumn{1}{@{}c@{}}{$\widehat{\AP}_q^s$}                                  \\
  \cline{2-2}    
          &                                                                      \\
  \phantom{\vdots}   &                                                                     \\
            &                                                                    \\
  \cline{2-2} 
          &                                                                      \\
  \phantom{\vdots}    &                                                                     \\
            &                                                                    \\
  \cline{2-2} 
  \phantom{\vdots}   &                                                                      \\
  \cline{2-2} 
          &                                                                      \\
  \phantom{\vdots}    &                                                                     \\
            &                                                                    \\
  \cline{2-2}
\end{tabular}
         & 
    \Large{$\longrightarrow$}
         & 
\begin{tabular}{ ll |c|}
         & \multicolumn{1}{c}{} & \multicolumn{1}{@{}c@{}}{$\AP^s_*$}             \\
  \cline{3-3}    
  $s_1$  & $t_1$                & \cellcolor[gray]{0.8}                         \\
  \vdots & \vdots               & \cellcolor[gray]{0.8}                         \\
  $s_m$  & $t_1$                & \cellcolor[gray]{0.8}                         \\
  \cline{3-3} 
  $s_1$  & $t_2$                &                                               \\
  \vdots & \vdots               &                                               \\
  $s_m$  & $t_2$                &                                               \\
  \cline{3-3} 
  \vdots & \vdots               &                                               \\
  \cline{3-3} 
  $s_1$  & $t_n$                &                                               \\
  \vdots & \vdots               &                                               \\
  $s_m$  & $t_n$                &                                               \\
  \cline{3-3} 
\end{tabular}
\end{tabular}

==> img/IPM/Figs/APhat.tex <==
\begin{tabular}{ cc@{}c c@{}cc c c@{}c}
\begin{tabular}{ r| ccc| c |@{ }c@{}|}
  \multicolumn{1}{c}{}&\multicolumn{1}{c}{$t_1$}&$\cdots$&\multicolumn{1}{c}{$t_n$} &\multicolumn{1}{c}{}\\
  \cline{2-4} \cline{6-6}
  $s_1$&&& & &\\
           &&& & &\\
  $\vdots$&\multicolumn{3}{c|}{$\widehat{\AP}_1$} & & $\widehat{\MAP}_1$\\
          &&& & &\\
  $s_m$&&& & &\\
  \cline{2-4} \cline{6-6}
  \multicolumn{6}{c}{}\\
  \cline{2-4} 
&    \multicolumn{3}{c|}{$\widehat{\AAP}_1$} &   \multicolumn{2}{c}{}\\
    \cline{2-4}
\end{tabular}
&
\ldots
&
\begin{tabular}{ r| ccc| c |@{ }c@{}|}
  \multicolumn{1}{c}{}&\multicolumn{1}{c}{$t_1$}&$\cdots$&\multicolumn{1}{c}{$t_n$} &\multicolumn{1}{c}{}\\
  \cline{2-4} \cline{6-6}
  $s_1$&&& & &\\
           &&& & &\\
  $\vdots$&\multicolumn{3}{c|}{$\widehat{\AP}_i$} & & $\widehat{\MAP}_i$\\
          &&& & &\\
  $s_m$&&& & &\\
  \cline{2-4} \cline{6-6}
  \multicolumn{6}{c}{}\\
  \cline{2-4} 
&    \multicolumn{3}{c|}{$\widehat{\AAP}_i$} &   \multicolumn{2}{c}{}\\
    \cline{2-4}
\end{tabular}
 &
\ldots
&
\begin{tabular}{ r| ccc| c |@{ }c@{}|}
  \multicolumn{1}{c}{}&\multicolumn{1}{c}{$t_1$}&$\cdots$&\multicolumn{1}{c}{$t_n$} &\multicolumn{1}{c}{}\\
  \cline{2-4} \cline{6-6}
  $s_1$&&& & &\\
           &&& & &\\
  $\vdots$&\multicolumn{3}{c|}{$\widehat{\AP}_q$} & & $\widehat{\MAP}_q$\\
          &&& & &\\
  $s_m$&&& & &\\
  \cline{2-4} \cline{6-6}
  \multicolumn{6}{c}{}\\
  \cline{2-4} 
&    \multicolumn{3}{c|}{$\widehat{\AAP}_q$} &   \multicolumn{2}{c}{}\\
    \cline{2-4}
\end{tabular}

  &
    \Large{$\longrightarrow$}
    &
    \begin{tabular}{ r| ccc| c |@{ }c@{ }|}
  \multicolumn{1}{c}{}&\multicolumn{1}{c}{$t_1$}&$\cdots$&\multicolumn{1}{c}{$t_n$} &\multicolumn{1}{c}{}\\
  \cline{2-4} \cline{6-6}
  $s_1$&\cellcolor[gray]{0.8}&& & &\\
           &\cellcolor[gray]{0.8}&& & &\\
  $\vdots$&\cellcolor[gray]{0.8}&$\widehat{\AP}_*$&\multicolumn{1}{c|}{} & & $\widehat{\MAP}_*$\\
          &\cellcolor[gray]{0.8}&& & &\\
  $s_m$&\cellcolor[gray]{0.8}&& & &\\
  \cline{2-4} \cline{6-6}
  \multicolumn{6}{c}{}\\
  \cline{2-4} 
&    \multicolumn{3}{c|}{$\widehat{\AAP}_*$} &   \multicolumn{2}{c}{}\\
    \cline{2-4}
\end{tabular}

\end{tabular}

==> img/IPM/Figs/MAPPrediction.tex <==
\begin{tabular}{ccc c ccc}
\begin{tabular}{ l |c|}
          \multicolumn{1}{c}{} & \multicolumn{1}{@{}c@{}}{$f_1$} \\
  \cline{2-2}    
  $s_1$               &                                               \\
  \vdots              &                                               \\
  $s_m$               &                                               \\
  \cline{2-2}
\end{tabular}
         & 
\begin{tabular}{@{}c@{}|c|}
 \multicolumn{1}{@{}c@{}}{}&\multicolumn{1}{@{}c@{}}{$f_i$}                                  \\
  \cline{2-2}    
          &                                                                      \\
  \phantom{\vdots}   &                                                                     \\
            &                                                                    \\
  \cline{2-2} 
\end{tabular}
         & 
\begin{tabular}{@{}c@{}|c|}
 \multicolumn{1}{@{}c@{}}{}&\multicolumn{1}{@{}c@{}}{$f_q$}                                  \\
  \cline{2-2}    
          &                                                                      \\
  \phantom{\vdots}   &                                                                     \\
            &                                                                    \\
  \cline{2-2} 
\end{tabular}
         & 
    \Large{$\longrightarrow$}
         & 
\begin{tabular}{ l |c|}
          \multicolumn{1}{c}{} & \multicolumn{1}{@{}c@{}}{$\widehat{\MAP}_*$}             \\
  \cline{2-2}    
  $s_1$               &                        \\
  \vdots              &                        \\
  $s_m$               &                        \\
  \cline{2-2} 
\end{tabular}
           & 
    \Large{$\Longleftrightarrow$}
         & 
\begin{tabular}{ l |c|}
          \multicolumn{1}{c}{} & \multicolumn{1}{@{}c@{}}{$\MAP$}             \\
  \cline{2-2}    
  $s_1$               &                        \\
  \vdots              &                        \\
  $s_m$               &                        \\
  \cline{2-2} 
\end{tabular}
\end{tabular}
